Membership Inference Attacks via Adversarial Examples

The raise of machine learning and deep learning led to significant improvement in several domains. This change is supported by both the dramatic rise in computation power and the collection of large datasets. Such massive datasets often include personal data which can represent a threat to privacy. Membership inference attacks are a novel direction of research which aims at recovering training data used by a learning algorithm. In this paper, we develop a mean to measure the leakage of training data leveraging a quantity appearing as a proxy of the total variation of a trained model near its training samples. We extend our work by providing a novel defense mechanism. Our contributions are supported by empirical evidence through convincing numerical experiments.

==> marple.tex <==
\subsection{Arclength of score function}

\textbf{Adversarial Path.} Consider a trained classifier $\hat f_{\theta}$ and a target sample $x \in \mathcal{X}$.
Using some adversarial attack, one may construct a new sample $\tilde x \in \mathcal{X}$ such that $\argmax{\hat f_{\theta}(x)} \neq \argmax{\hat f_{\theta}(\tilde x)}$.
In practice, this adversarial example is of the form $\tilde x = x + \varepsilon$ and is obtained by optimizing the gaussian noise $\varepsilon$ (citer ref attacks).
In the idea that training samples are associated to high peaks of the score function, it is natural to measure the arclength along the adversarial path connecting the target sample $x$ and the adversarial example $\tilde x$.
For that matter, consider the parameterization $\gamma_x: [0,1] \to \rset$ given by
\begin{align*}
    \gamma_x: t \mapsto \|\hat f_{\theta}(x + t \varepsilon)\|_{\infty}
\end{align*}
 and the associated arclength $\mathscr{L}(\gamma_x) = \int_{0}^1 |\gamma_x'(t)|\mathrm{d}t$.

 \textbf{Approximated Total Variation.} Consider a fixed integer $N \in \mathbb{N}$ and the partition sequence $0=t_1<\ldots<t_N=1$ given by $(t_k)_{k\leq N}$ given by $t_k = k/N$.
 We measure the arclength along the adversarial path using the approximation $\mathscr{L}_N(\gamma_x)$ given by
 \begin{align} \label{eq:approx_tv}
     \mathscr{L}_N(\gamma_x) = \sum_{k=1}^N |\gamma_x(t_{k})-\gamma_x(t_{k-1})|
 \end{align}
 Note that with Riemann sums, we have $\mathscr{L}_N(\gamma_x) \to \mathscr{L}(\gamma_x)$ as $N \to +\infty$.


==> preliminaries.tex <==
\subsection{Statistical Learning}

\subsection{Learning with noisy labels}
The authors of \cite{natarajan2013learning} introduce the framework of learning with noisy labels.

\subsection{Adversarial Attacks}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/illustration.pdf}
    \caption{Illustration of adversarial examples (red stars) resulting from train data (blue circle). The background color represents the probability output of a binary classifier.}
    \label{fig:my_label}
\end{figure}

\subsection{Membership Inference Attack}

\subsection{Arc length and total variation}

For any real-valued continuous function $f$ defined on an interval $I \subset \rset$, the total variation is a measure of the one-dimensional arc length of the curve with parametric equation $t \mapsto f(t)$ for $t \in I$. More precisely, 
\begin{definition}[Total variation for univariate function $\rset$] Consider a real-valued function $f$ defined on an interval $[a,b] \subset \rset$ and denote by $\Pi$ the set of all partitions $\Pi = \{\pi = (x_{0},\ldots,x_n) | a=x_0 < \ldots < x_n=b \}$ of the given interval. The total variation of $f$ on $[a,b]$ is given by
\begin{align*}
V_{[a,b]}(f) = \sup_{\pi \in \Pi} \sum_{k=1}^{n} |f(x_{k}) - f(x_{k-1})|.
\end{align*}
Moreover, if $f$ is differentiable, we have
\begin{align*}
    V_{[a,b]}(f) = \int_{a}^b |f'(t)|\mathrm{d}t.
\end{align*}
\end{definition}

%Given an input point $x \in \mathcal{X}$ (an image) with label $y \in \mathcal{Y}$ and its predicted label $f(x)$, we can use an adversarial attack to build an image $\tilde x = x + \varepsilon$ such that $f(x) \neq f(\tilde x)$. Idea from \cite{Grosso2022LeveragingAE}: compute the distance $d(x,\tilde x) \approx \|\varepsilon\|$ with the following intuition :
%\begin{itemize}
%    \item if $\|\varepsilon\|$ is big then it is more likely that the input image $x$ belongs to the training set (since overconfidence on train, we need to add lot of noise to misclassify !)
%\end{itemize}
%In this paper, we no longer focus on the distance computed on the input space but rather we observe the classifier's output variation induced along the \emph{adversarial path}. This observed quantity corresponds to a proxy of the total variation of the softmax classifier output on the interest interval. 


%Given a length $n$ of the adversarial path and its associated precision $1/n$, we define the adversarial path as the sequence $x_0 = x , x_1, \ldots,x_n= \tilde x$ where $x_k = x + k \varepsilon/n$. The quantity of interest is
%\begin{align*}
%    \Delta_n(x,\tilde x) = \sum_{k=0}^{n-1}, |f(x_{k+1}) - f(x_{k})|
%\end{align*}
%which appears to be upper-bounded by the total variation of $f$ on the domain 

Given a classifier $f \in \mathcal{G}$, an input sample $x \in \mathcal{X}$ and its associated adversarial example $\tilde x \in \mathcal{X}$, any general membership inference attack strategy may be written using a functional $\varphi: \mathcal{G} \times \mathcal{X} \times \mathcal{X} \to \rset$ as $\un\{\varphi(f,x,\tilde x) \geq \tau\}$. For instance, \citet{Grosso2022LeveragingAE} considered different distances associated to the norms $\ell_1,\ell_2$ and $\ell_\infty$ by taking $\varphi(f,x,\tilde x) = \|\tilde x - x\|$. Such distances are only concerned by the input space $\mathcal{X}$ and do not use the classifier $g$. Based on the several remarks concerning Figure (TO do figure 3d), we argue that more attention is needed on the output space as the landscape is more likely to capture the high confidence levels associated to the samples that were used during training.


==> synthetic.tex <==
In this section, our goal is to provide further insight into the importance of exploiting local \textit{peaks of confidence} of the classifier to perform membership inference of training data.
This motivates and provides further theoretical understanding of the MIA strategy detailed in \cite{Grosso2022LeveragingAE} and depicted in Section~\ref{sec:experiments}.
Indeed, the key intuition is the following: Close to its training samples more noise should be required to fool a classifier, because the sample needs to step further away from the local excesses of confidence.
We work with simulated data in order to maintain a controlled environment. 
 %We perform a 2 sample Kolmogorov-Smirnov test to confirm that both distributions are significantly different 
%Some adversary random noise, controlled by a parameter $\kappa$ is added to the data samples from both the train and  test sets.
% We perform 2 sample Kolmogorov Smirnov tests on the maximum probability provided by the classifier on the pair $\big(\mathcal{D}_{train}, \mathcal{D}_{train}^\prime \big)$. Then we perform the same statistical test on the classifier's output on the test set and its noisy counterpart  $\big(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime \big)$. 

First, we start by describing our experimental framework.
Both train and test datasets are generated as follows.
We generate ${n =5 \cdot 10^3}$ copies $X_1, \ldots, X_n$ of a bivariate sample $X$ from different  mixtures of Gaussians {through \texttt{make\_classification} function from Scikit-learn} \cite{pedregosa2011scikit}.
Each sample $X_i$ gets a corresponding label $Y_i \in \mathcal{Y}$ where $i \leq n$ and $\mathcal{Y}$ is a discrete and finite label set.
Data from different clusters (\textit{i.e.} modes of the Gaussian mixtures) are labeled differently and classes are balanced.
A multi layer perceptron $\widehat{g}_\theta$ is trained on the training set $\mathcal{D}_{\text{train}} = \{(X_i, Y_i)\}_{1 \leq i \leq n}$.
A second dataset, $\mathcal{D}_{\text{test}}$ {with the same size $n=5 \cdot 10^3$ as $\mathcal{D}_{\text{train}}$} is generated similarly to $\mathcal{D}_{\text{train}}$ and shares the same size $n$ with $n=5 \cdot 10^3$.
The average pairwise intra-cluster distance is computed.
We denote by $\mu^y_{\text{train}}$ the average pairwise distance for data samples from the subset of the train set labeled $y \in \mathcal{Y}$.
We denote by $\mu^y_{\text{test}}$ the counterpart of $\mu^y_{\text{train}}$ for the test set.
In short, the pairwise distance for data of $\mathcal{D}_\delta$ labeled $y$ is computed as follows,
\begin{equation}
    \mu^y_\delta = \frac{1}{|\mathcal{D}_\delta|}\sum_{\substack{i=2, \\ j < i}}^{|\mathcal{D}_{\delta}|} \|X_i - X_j\|_2^2 \, \un\{Y_i = Y_j = y\},
\label{eq:mu}
\end{equation}
where $y \in \mathcal{Y}$, $\delta \in \{\text{train}, \text{test}\}$. 

We will now study two possible settings regarding the random noise added to the data points belonging to the train and test sets.
First, in \ref{subsubsec:nonisotropicgaussiannoise}, we study the setting where the random noise is non-isotropic and directed towards the empirical barycenter of the closest class that is differently labeled.
In \ref{subsubsec:isotropicgaussiannoise}, we consider the setting { where the random noise is} isotropic Gaussian noise.

\subsection{Non-Isotropic Noise}
\label{subsubsec:nonisotropicgaussiannoise}
%Experiments and results from Section~\ref{sec:experirements} on simulated data are further detailed and enhanced here.\\

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv4_truncated.pdf}
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv_purpleyellow4.pdf}
\caption{(Left) Boxplot of univariate two sample Kolmogorov-Smirnov tests average $p$-values between max scores provided by $\widehat{g_\theta}$ computed on the original train data $\mathcal{D}_{\text{train}}$, (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$.
(Right) Boxplot of bivariate two sample Kolmogorov-Smirnov tests average $p$-values between the original train data $\mathcal{D}_{\text{train}}$ (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$. The boxplots display the results for $100$ different (random) iterations of the experiment. The number of classes is equal to 4.}
    \label{fig:boxplots4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv3_truncated.pdf}
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv_purpleyellow3.pdf}

\caption{(Left) Boxplot of univariate two sample Kolmogorov-Smirnov tests average $p$-values between max scores provided by $\widehat{g_\theta}$ computed on the original train data $\mathcal{D}_{\text{train}}$, (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$.
(Right) Boxplot of bivariate two sample Kolmogorov-Smirnov tests average $p$-values between the original train data $\mathcal{D}_{\text{train}}$ (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$. The boxplots display the results for $100$ different (random) iterations of the experiment. The number of classes is equal to 3.}
    \label{fig:boxplots3}
\end{figure}

Let $\varepsilon_i^{y, \delta}$ be a univariate Gaussian noise centered at $0$ and with standard deviation $\sigma^y_\delta$  defined as follows $\sigma^y_\delta = \kappa \mu^y_\delta$, where $\kappa \geq 0 $ is a noise control factor, $\delta \in \{\text{train}, \text{test}\}$ and $y \in \mathcal{Y}$. Let us now define the noisy datasets $\mathcal{D}_{\text{train}}^\prime$ and $\mathcal{D}_{\text{test}}^\prime$.
For any sample $X_i$, belonging to $\mathcal{D}_{\delta}$ labeled $y$, we create a corresponding sample $X_i^\prime$ defined as follows:
\begin{equation}
    X_i^\prime = X_i + |\varepsilon_i^{y, \delta}| u_i,
    \label{eq:noisy_data_}
\end{equation}
where $u_i$ represents the normalized vector from $X_i$ and directed towards the barycenter of the closest class differently labeled.


$X_i^\prime$ defined in Equation~\ref{eq:noisy_data_} belongs to the noisy dataset $\mathcal{D}_{\delta}^\prime$. The greater $\kappa$, the greater the intra-class difference between $\mathcal{D}_{\delta}$ and $\mathcal{D}_{\delta}^\prime$.
In this way, one can control the amount of noise within each class without necessarily disrupting \added[id=GP]{How do you disrupt? In what sense?} the whole dataset.
Four times, we perform two sample Kolmogorov-Smirnov tests \added[id=GP]{cite?} on data for each class: a first univariate test between the max probability output of the classifier $\widehat{g}_\theta$ on the data from pairs $\big(\mathcal{D}_{\text{train}}, \mathcal{D}_{\text{train}}^\prime\big)$ and $\big(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime\big)$ and a second multivariate two sample Kolmogorov Smirnov test (see \cite{fasano1987multidimensional}) directly computed on data from the same pairs $\big(\mathcal{D}_{\text{train}}, \mathcal{D}_{\text{train}}^\prime\big)$ and   $\big(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime\big)$. The $p$-values are averaged over the total number of classes in their respective pairs $\big(\mathcal{D}_{\text{train}}, \mathcal{D}_{\text{train}}^\prime\big)$ or   $\big(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime\big)$. 

%Figure~\ref{} extends the results from Figure~\ref{} on a wider range of noise parameter $\kappa$.

Figure~\ref{fig:boxplots4} (\textit{respectively} Figure~\ref{fig:boxplots3}) (Left) depicts the evolution of $p$-values from the two-sample Kolmogorov-Smirnov tests performed on the max output of the classifier $\widehat{g}_\theta$ where the number of classes is equal to 4 (\textit{respectively} equal to 3).
Regarding the classifier output, as more noise is added, the distributional gap is more remarkable between the original training data and their noisy counterpart than compared to the test data and their noisy counterpart, as suggested by the lower average $p$-values for the pair $\big(\mathcal{D}_{\text{train}}, \mathcal{D}_{\text{train}}^\prime\big)$ compared to  $\big(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime\big)$. The boxplots on the right (\textit{respectively} Figure~\ref{fig:boxplots3} (Right)) provide the evolution of the $p$-values from a bivariate two-sample Kolmogorov-Smirnov test directly computed on the input data, it describes the evolution of the distributional influence of the noise parametrized by $\kappa$.
As more noise is added (\textit{i.e.} the larger $\kappa$), the larger is the difference between the original data and their noisy counterparts. Hence, the smaller are the $p$-values regarding the train and test sets and their respective noisy counterparts. 
The decay rate with $\kappa$ of $p$-values is similar between $(\mathcal{D}_{\text{train}}, \mathcal{D}_{\text{train}}^\prime)$ and $(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime)$. 
The dashed line represents the $5\%$ value, thus for a noise level $\kappa$ greater than $0.1$ it is not guaranteed that the noisy data is not significantly different from the original data.   

%\clearpage
\subsection{Isotropic Gaussian Noise}
\label{subsubsec:isotropicgaussiannoise}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv3_truncated_non_adversarial.pdf}
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv_purpleyellow_non_adversarial3.pdf}

\caption{(Left) Boxplot of a univariate two sample Kolmogorov-Smirnov test $p$-values average over all classes between max scores provided by $\widehat{g_\theta}$ computed on the original train data $\mathcal{D}_{\text{train}}$, (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$.
(Right) Boxplot of a bivariate two sample Kolmogorov-Smirnov test $p$-values between the original train data $\mathcal{D}_{\text{train}}$ (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$. The boxplots display the results for $100$ different (random) generations of data. The number of classes is equal to 3.}
    \label{fig:boxplots3_non_adversarial}
\end{figure}

\begin{figure}[th!]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv4_truncated_non_adversarial.pdf}
    \includegraphics[width=0.45\textwidth]{figures/toydata_violinplot_long_adv_purpleyellow_non_adversarial4.pdf}

\caption{(Left) Boxplot of a univariate two sample Kolmogorov-Smirnov test $p$-values average over all classes between max scores provided by $\widehat{g_\theta}$ computed on the original train data $\mathcal{D}_{\text{train}}$, (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$.
(Right) Boxplot of a bivariate two sample Kolmogorov-Smirnov test $p$-values between the original train data $\mathcal{D}_{\text{train}}$ (\textit{respectively} test data $\mathcal{D}_{\text{test}}$) and the noisy train counterpart $\mathcal{D}_{\text{train}}^\prime$ (\textit{respectively} noisy test counterpart $\mathcal{D}_{\text{test}}^\prime$)  with varying noise level $\kappa$. The boxplots display the results for $100$ different (random) generations of data. The number of classes is equal to 4.}
    \label{fig:boxplots4_non_adversarial}
\end{figure}


In this section, we perform a similar experiment to the one conducted in Section~\ref{subsubsec:nonisotropicgaussiannoise} with a simpler setting, the noise is no longer adversarial but an isotropic quantity. 

Let $\varepsilon_i^{y, \delta}$ be a bivariate Gaussian noise centered in $0$ and with covariance matrix $\Sigma^y_\delta = \kappa \mu^y_\delta \mathbf{I}$, where $\mathbf{I}$ denotes the $2\times2$ identity matrix, $\mu_\delta^y$ is defined in Equation~\ref{eq:mu} ,  $\kappa$ remains the noise control factor, $y \in \mathcal{Y}$ is a given class of the label set and we recall  that $\delta \in \{\text{train}, \text{test}\}$. Similarly to Section~\ref{subsubsec:nonisotropicgaussiannoise}, we define the noisy datasets $\mathcal{D}_{\text{train}}^\prime$ and $\mathcal{D}_{\text{test}}^\prime$. For any sample $X_i$, belonging to $\mathcal{D}_{\delta}$, labeled $\sigma 1$, we create a corresponding sample $X_i^\prime$ defined as follows,
\begin{equation}
    X_i^\prime = X_i + \varepsilon_i^{y, \delta}, 
    \label{eq:noisy_data}
\end{equation}
where $y \in \mathcal{Y}$, and $\delta \in \{\text{train}, \text{test}\}$.

$X_i^\prime$ defined in Equation~\ref{eq:noisy_data} belongs to the noisy dataset $\mathcal{D}_{\delta}^\prime$.
The greater $\kappa$, the greater the intra-class difference between $\mathcal{D}_{\delta}$ and $\mathcal{D}_{\delta}^\prime$.
In this way one can control the amount of noise within each class without necessarily disrupting the whole dataset.
We perform the same statistical tests. Same conclusions than Section~\ref{subsubsec:nonisotropicgaussiannoise} can be obtained regarding the isotropic noise setting, based on Figure~\ref{fig:boxplots3_non_adversarial} and Figure~\ref{fig:boxplots4_non_adversarial}.
Figure~\ref{fig:boxplots3_non_adversarial} (Left) and Figure~\ref{fig:boxplots4_non_adversarial} (Left) transcribe local pics of confidence of the classifier on train data.
Regarding the classifier output, as more isotropic noise is added, the distributional gap is more remarkable between the original training data and their noisy counterpart when compared to the test data and their noisy counterpart, as suggested by the lower average $p$-values for the pair $\big(\mathcal{D}_{\text{train}}, \mathcal{D}_{\text{train}}^\prime\big)$ compared to  $\big(\mathcal{D}_{\text{test}}, \mathcal{D}_{\text{test}}^\prime\big)$.
Figure~\ref{fig:boxplots3_non_adversarial} (Right) and Figure~\ref{fig:boxplots4_non_adversarial} (Right) provide the evolution of the $p$-values on a bivariate two-sample Kolmogorov-Smirnov test. The dashed line represents the $5\%$, For all noise level $\kappa$ considered, we can reject the hypothesis that the noisy data is not significantly different from the original data reinforcing the adversarial distance strategy depicted in Section~\ref{sec:MembershipInferenceAttacksfromAdversarialExamples}.   

%We perform a multivariate Kolmogorov-Smirnov \cite{fasano1987multidimensional} test on the data $X_is$ and their noisy counterparts $X_i^\prime s$.
\subsection{Conclusion on Experimental Findings on Simulated Data}
While adding an isotropic Gaussian noise induces less remarkable change to the multivariate input data, the naive adversarial noise leads to more remarkable change regarding $p$-values for both univariate and multivariate Kolmogorov-Smirnov test. 
Eventually, on both experimental designs we observed that the influence of the added noise on the classifier max score is greater on train data compared to test data.
